Exploitation Techniques and Defenses for Data-Oriented Attacks

Data-oriented attacks manipulate non-control data to alter a program's benign behavior without violating its control-flow integrity. It has been shown that such attacks can cause significant damage even in the presence of control-flow defense mechanisms. However, these threats have not been adequately addressed. In this SoK paper, we first map data-oriented exploits, including Data-Oriented Programming (DOP) attacks, to their assumptions/requirements and attack capabilities. We also compare known defenses against these attacks, in terms of approach, detection capabilities, overhead, and compatibility. Then, we experimentally assess the feasibility of a detection approach that is based on the Intel Processor Trace (PT) technology. PT only traces control flows, thus, is generally believed to be not useful for data-oriented security. However, our work reveals that data-oriented attacks (in particular the recent DOP attacks) may generate side-effects on control-flow behavior in multiple dimensions, which manifest in PT traces. Based on this evaluation, we discuss challenges for building deployable data-oriented defenses and open research questions.

==> Makefile <==
#!/usr/bin/make -f
# A Makefile for building LaTeX documents.
#
# Thomas Nyman <thomas.nyman@aalto.fi>

### Configuration section ###

# Tools
TYPESETTER ?= pdflatex
BIBTEX ?= bibtex
VIEWER ?= evince

# Flags
LATEXFLAGS ?= -file-line-error

# Directories
BASEDIR ?= .
DESTDIR ?= ${BASEDIR}/
SRCDIR  ?= ${BASEDIR}/
INCLDIR ?= ${BASEDIR}/sections/

# Files
DOCUMENT ?= $(wordlist 1, 1, $(sort $(basename $(notdir $(filter-out %bst.tex, $(wildcard ${SRCDIR}/*.tex))))))
INCLUDES ?= $(wildcard ${INCLDIR}/*.tex)

# Alternate document expansions
ABBRDOCUMENT = "\def\isabridged{1} \input{$(DOCUMENT).tex}"
ANONDOCUMENT = "\def\isanonymous{1} \input{$(DOCUMENT).tex}"

# Targets for cleaning
MOSTLYCLEANFILES = \
	${DESTDIR}/*.aux \
	${DESTDIR}/*.log \
	${DESTDIR}/*~

CLEANFILES = ${MOSTLYCLEANFILES} \
	${DESTDIR}/*.bbl \
	${DESTDIR}/*.blg \
	${DESTDIR}/*.glo \
	${DESTDIR}/*.gls \
	${DESTDIR}/*.glg \
	${DESTDIR}/*.idx \
	${DESTDIR}/*.ind \
	${DESTDIR}/*.ilg \
	${DESTDIR}/*.lof \
	${DESTDIR}/*.lot \
	${DESTDIR}/*.nav \
	${DESTDIR}/*.out \
	${DESTDIR}/*.snm \
	${DESTDIR}/*.toc \
	${DESTDIR}/*.dvi \
	${DESTDIR}/*.ps

DISTCLEANFILES = ${CLEANFILES} \
	${DESTDIR}/${DOCUMENT}.pdf

# Make sure DESTDIR exists
# Note: defining a separate rule for DESTDIR as a dependency for pdf files
# might seem cleaner, but won't work since the modification time of the
# directory is changed as output files are created.
$(shell [ -d "${DESTDIR}" ] || mkdir -p ${DESTDIR})

# Make sure the destination directory is set for the typesetter
override LATEXFLAGS += -output-directory=${DESTDIR}

### Targets ###

build: $(DOCUMENT)

# Display document in preferred document viewer
show: $(DOCUMENT)
	$(VIEWER) ${DESTDIR}/${DOCUMENT}.pdf &

# Typeset document and resolve table of contents
toc:
	${TYPESETTER} ${LATEXFLAGS} $(DOCUMENT)
	${TYPESETTER} ${LATEXFLAGS} $(DOCUMENT)

# Typeset document and resolve bibliography references
bib:
	${TYPESETTER} ${LATEXFLAGS} $(DOCUMENT)
	${BIBTEX}     $(DOCUMENT)
	${TYPESETTER} ${LATEXFLAGS} $(DOCUMENT)
	${TYPESETTER} ${LATEXFLAGS} $(DOCUMENT)

# Typeset abridged version of document
abridged: 
	${TYPESETTER} ${LATEXFLAGS} ${ABBRDOCUMENT}
	${BIBTEX}     $(DOCUMENT)
	${TYPESETTER} ${LATEXFLAGS} ${ABBRDOCUMENT}
	${TYPESETTER} ${LATEXFLAGS} ${ABBRDOCUMENT}

# Typeset anonymous version of document
anonymous:
	${TYPESETTER} ${LATEXFLAGS} ${ANONDOCUMENT}
	${BIBTEX}     $(DOCUMENT)
	${TYPESETTER} ${LATEXFLAGS} ${ANONDOCUMENT}
	${TYPESETTER} ${LATEXFLAGS} ${ANONDOCUMENT}

### Housekeeping rules ###

mostlyclean:
	${RM} ${MOSTLYCLEANFILES}

clean:
	${RM} ${CLEANFILES}

distclean:
	${RM} ${DISTCLEANFILES}

### Special targets ###

# These rules define basename (without suffix) targets and sets up
# corresponding relative path targets as dependencies.
.SECONDEXPANSION:
${DOCUMENT}: $(DESTDIR)/$$@.pdf

# Targets to be run unconditionally
.PHONY: mostlyclean clean distclean

### Implicit rules ###

${DESTDIR}/%.pdf: ${SRCDIR}/%.tex ${INCLUDES}
	${TYPESETTER} ${LATEXFLAGS} $<



==> sections/05-detectabilityanalysis.tex <==
\subsection{Can PT be used to detect data-oriented attacks?} \label{sec3:ptdoa}
%When Data-oriented Attacks Meet PT
%In this section, we provide an in-depth understanding of data-oriented attacks in terms of the anomalous program behavior detection. 
%Though PT is generally believed to be not useful for data-oriented security since it only traces control-flows, 
%we show that data-oriented attacks may generate side-effects on control-flow behaviors in multiple dimensions, which are manifested in PT traces. 
We discuss different cases where PT can or cannot help detect data-oriented attacks. 
The \textit{necessary condition} for detecting a data-oriented attack using control-flow tracing is that, the attack directly or indirectly affects the flow of a program's execution. 
%At first glance it seems unlikely to use PT to detect DOA anomalies. However, XXX
%\subsection{Motivations}
Typically, uses of non-control data in a program can be classified either as predicate uses or non-predicate uses (such as computation uses). A predicate-use directly affects the control-flow. While a non-predicate use may affect the computation or the output of a program~\cite{Rapps:1985:TSE}.
%They proposed to detect infeasible/invalid control-flow paths caused by attacks at run-time via constructing correlations among branches at compile-time. However, the proposed approach is restricted to simple forms of conditional predicates, \eg, comparing a variable with a constant value. 
%numerical comparisons. since it is difficult to symbolically evaluate the "subsume" relationship between predicates. 
%It is challenging to statically determine branch correlations with arbitrary predicate expressions, especially for predicates with indirect data dependency or involving function calls. 
Though data-oriented attacks do not violate control-flow integrity, Zhuang~\etal~\cite{Zhuang:MICRO:2006} showed that many non-control data attacks actually cause changes in control-flows. In their experiments, on average 49.4\% of memory tamperings change program control-flows. 

\textbf{Detectable cases:} we observe that data-oriented attacks can potentially cause three types of anomalous control-flow behaviors. 
\begin{enumerate}[*] %impact of continuous buffer overflowing. 
	\item \emph{Incompatible branch behavior}: Manipulating a predicate-use variable (\eg, decision-making data) can change the default branch behavior of a program.  %and there is no write to the manipulated variable between these two branch sites (\ie, without an intervening assignment)
	If there exist two correlated conditional branches that are data-dependent on the manipulated variable before and after the data manipulation site, it is likely the data manipulation incurs incompatible branch behaviors that can be detected by control-flow tracing. 
	Such anomalies occur in Stage S3 of data-oriented attacks (\ie, when a corrupted variable is used). 
	We observe such an incompatible branch behavior in the the decision-making data attack shown in Listing~\ref{lst:authen}.
	On the other hand, continuous buffer overflow may generate side effects on control-flow behavior, which could result in an incompatible control-flow path observable in Stage S2. For example, though the target buffer is not used for predicate-use, some decision-making variables close to the buffer may be inevitably corrupted. We manually analyzed 14 vulnerable programs in a test suite for buffer overflows~\cite{SRD}, and found that 5 out of 14 overflows cause side impacts on decision-making variables (\ie, involved in predicate expressions). 
	In Section~\ref{sec5:feasibility}, we demonstrate the feasibility of exploring branch correlation to detect incompatible branch behaviors. We successfully detect an incompatible branch behavior in the ProFTPd DOP attack~\cite{Hu:2015:DOA}, where details can be found in Section~\ref{sec5:branchbehavior}.
	%irrelevant to achieve the attack purpose,
	\item \emph{Micro-level control-flow frequency anomaly}: Short control-flow paths may exhibit unusual execution frequencies. For instance, corrupting variables which directly or indirectly control loop iterations cause such frequency anomalies.
	Micro-level control-flow frequency anomalies may be observed in different stages of data-oriented attacks. In addition, control-flow bending (CFB) attacks~\cite{Carlini:2015:CBE} and resource wastage attacks~\cite{Baliga:2007:SP} may also lead to unusual control-flow frequencies.
	%[???point example of Code2???]
	% such as repeatedly corrupting variables to achieve the attack purpose and avoid segmentation faults
	%The control-flow bending (CFB\footnote{CFB is a generalization of non-control-data attacks. It allows modifications of control data so long as the modified indirect branch targets are valid as defined by a CFI policy.}) attacks~\cite{Carlini:2015:CBE} may also lead to unusual control-flow frequencies. 
	\item \emph{Interaction frequency anomaly (macro-level frequency anomaly)}:	In an interactive DOP attack, an attacker interacts with a vulnerable program to repeatedly corrupt variables to achieve the attack purpose and avoid segmentation faults. This inevitably results in frequency anomalies during the client-server interaction, which can also be captured by control-flow tracing. For example, in the ProFTPd DOP attack introduced in Section~\ref{sec2}, an attacker needs to send a large number of FTP commands with malicious inputs to the ProFTPd server to corrupt the program memory repeatedly.  
	%In particular, DOP attacks usually involve multiple interactions between an attacker and the vulnerable program~\cite{Hu16}. Such frequency anomalies can be captured by control-flow tracing. In addition, resource wastage attacks~\cite{Baliga:2007:SP} may also cause control-flow frequency anomalies. 
	%or network traffic tracing
\end{enumerate}

\textbf{Undetectable cases:} Detecting data-oriented attacks using control-flow tracing requires that an attack manifests incompatible/unusual control-flow behaviors, either incompatible branch behaviors or frequency anomalies. When a manipulated variable is only used for computation or output (\ie, non-predicate use), and the exploit does not incur any side effect on control transfers, such an attack is undetectable by PT-base control-flow tracing. We list typical undetectable cases, which are mainly direct data manipulation (DDM) attacks. 
\begin{enumerate}[$\diamond$]
	\item Corrupting user identity for privilege escalation: Simply corrupting a user identify data (\eg, \texttt{UID}) may lead to  
	a compromise of the root privilege. However, for an undetectable data manipulation with the privilege escalation, an attacker usually goes after malicious actions once obtaining the new privilege, \eg, launching a shell. Such malicious actions can be easily detected by control-flow tracing.
	\item Corrupting configuration data: Corrupting configuration data via format string vulnerabilities may evade PT-based detection, since format string vulnerabilities allow a single memory write without a side effect on control-flow behavior.
	\item Constructing exfiltration channels for information leakage: Attackers exploit an existing information outlet (also known as sink such as \texttt{printf} or \texttt{send} functions) for information leakage by replacing the pointer value of the outlet function's parameter with the address of the data to be exfiltrated. Such an attack may not incur any anomalous control-flow behavior. 
\end{enumerate}




==> sections/10-implementation.tex <==
% vim:ft=tex:

\section{Implementation}


\subsection{The ProFTP attack implementation}

\todo[inline]{HL: This is just a placeholder. Section or subsection can be moved as needed.}

To evaluate DOP-attach characteristics we have ported the original ProFTP attack~\cite{Hu16} to a custom Ubuntu 16.04 setup.
Due to library and memory layout changes some modifications were required.
The attack target --- the RSA private exponent --- is beyond several dereferences and must be correctly dereferenced in order to avoid memory faults.
The various DOP gadgets also rely on specific memory addresses, including a byte map to in-memory bytes with the values $\mathrm{00}$ to $\mathrm{ff}$.

Because the attack exploits the \texttt{sreplace} string manipulation function many of the gadgets are affected by the peculiarities of C strings.
For instance, memory dereference is done using string substitution in \texttt{sreplace}.
However, if the address contains a zero byte --- the C string terminator--- the written address will be prematurely cut.
To accommodate these nuances and automate memory address locating we modified the original metasploit module and created an automated script to scan the ProFTP binary.


==> sections/99-readme.tex <==
\section{Makefile}

The included Makefile provides targets for typesetting a PDF of the source document. It also provides targets to typeset abridged or anonymous version a document based on the \texttt{\textbackslash ifabridged} and \texttt{\textbackslash ifanonymous} conditionals. Negated conditionals \texttt{\ifnotabridged} and \texttt{\ifnotanonymous} are also provided.

\subsection{Makefile Targets and Variables} 

\paragraph{\texttt{show}} The default. Displays the typeset document in the viewer of choice, running the source document through the typesetter if needed.  See the description of the DOCUMENT, TYPESETTER and VIEWER variables for information on how to adjust the document, typesetter or viewer.  

\paragraph{\texttt{toc}} Typesets the document and resolves the table of contents.

\paragraph{\texttt{bib}} Typesets the document and resolves bibliography references.

\paragraph{\texttt{abridged}} Typesets abridged version of document.

\paragraph{\texttt{anonymous}} Typesets anonymous version of document.

\paragraph{\texttt{mostlyclean}} Delete the auxiliary and log file in the output directory that are normally created by typesetting the document.  

\paragraph{\texttt{clean}} Delete all intermediate files in the output directory that are normally created by running the typesetter. However, don’t delete the typeset document.

\paragraph{\texttt{distclean}} Clean all files in the destination directory (or created by this makefile) that are created by running the typesetter program. If you have checked out the source from version control and typeset the document without creating any other files, ‘make distclean’ should leave only the files that were checked into the VCS.

\subsection{Variables within the Makefile}

These variables may be adjusted on the \texttt{make} command line to influence the behaviour of the Makefile target. For instance, to typeset \texttt{mydocument.tex} in the current directory invoke \texttt{make} as follows:

\begin{verbatim}
$ make DOCUMENT=mydocument
\end{verbatim}

\paragraph{\texttt{TYPESETTER}} Path to the typesetter. Defaults to \texttt{pdflatex}.

\paragraph{\texttt{BIBTEX}} Path to \texttt{bibtex}. Defaults to \texttt{bibtex}.

\paragraph{\texttt{VIEWER}} Path to the viewer of choice. Defaults to \texttt{evince}.

\paragraph{\texttt{LATEXFLAGS}}  Command line flags passed to the typesetter. You can add flags to \texttt{LATEXFLAGS} by setting the variable on the \texttt{make} command line, but you cannot set the destination directory this way. To adjust the destination directory, set the DESTDIR variable. Defaults to \texttt{-file-line-error}.  

\paragraph{\texttt{DESTDIR}} Path to the destination directory. Defaults to the current directory.

\paragraph{\texttt{SRCDIR}} Path to source directory. Defaults to the current directory.

\paragraph{\texttt{INCLDIR}} Path to the directory included LaTeX files should be searched for. Defaults to \texttt{./sections}.

\paragraph{\texttt{DOCUMENT}} The name of the document to typeset (without file extension). Defaults to the basename of the first file (in alphabetical order) with \texttt{.tex} extension.

\paragraph{\texttt{INCLUDES}} List of included LaTeX files. Defaults to files found in the \texttt{INCLDIR} path.

\paragraph{\texttt{MOSTLYCLEANFILES}} List of glob patterns defining which files are removed on \texttt{make mostlyclean}.

\paragraph{\texttt{CLEANFILES}}  List of glob patterns defining which files are removed on \texttt{make clean}.

\paragraph{\texttt{DISTCLEANFILES}} List of glob patterns defining which files are removed on \texttt{make distclean}.


